Group testing for overlapping communities

In this paper, we propose algorithms that leverage a known community structure to make group testing more efficient. We consider a population organized in connected communities: each individual participates in one or more communities, and the infection probability of each individual depends on the communities (s)he participates in. Use cases include students who participate in several classes, and workers who share common spaces. Group testing reduces the number of tests needed to identify the infected individuals by pooling diagnostic samples and testing them together. We show that making testing algorithms aware of the community structure, can significantly reduce the number of tests needed both for adaptive and non-adaptive group testing.

==> algorithm-2stage.tex <==
\begin{algorithm}
	\caption{Two-stage Testing}
	\label{algorithm-2stage} 
	%$\testmatrix_1'$ of size $\nTests_1\times \nFamilies$ is the testing matrix identifying community infection status in Stage 1. \\
	%$\testmatrix_2'$ of size $\nTests_2\times |\GroupTestItemSet|$ is the testing matrix for group testing in Stage 2. \\
	$\GroupTest2()$ gives the testing result of group testing a set of members. \\
	$\IndividualTest2()$ gives the testing result of individually testing a set of members. \\
	$\MemberInclusionSet(i)$ is the set of communities that include member $i$. \\
	$\GroupTestItemSet$ is the set of  members to be group tested in Stage 2. \\
	$\IndividualTestItemSet$ is the set of  members to be individually tested in Stage 2. \\
	$\hat{\FamilyTestResult}_i$ is the estimated infection status of community $i$ (1 for ``positive'' and 0 for ``negative'').\\
	$\hat{\defVariable}_i$ is the estimated infection status of member $i$ (1 for ``positive'' and 0 for ``negative'').
	\begin{algorithmic}[1]
		\State{$\left[\hat{\FamilyTestResult}_1,\cdots,\hat{\FamilyTestResult}_{\nTests_1}\right]=\GroupTest2([1:\nFamilies])$}
		\State{Set $\GroupTestItemSet=\emptyset$}
		\State{Set $\IndividualTestItemSet=\emptyset$}
		\For {$i\in[1:\nItems]$}
		\If{$\sum(\hat{\FamilyTestResult}_j:~j\in\mathit{MemberInclusionSet}(i))==0$}
		\State{$\GroupTestItemSet\leftarrow\GroupTestItemSet\cup\{i\}$}
		\Else
		\State{$\IndividualTestItemSet\leftarrow\IndividualTestItemSet\cup\{i\}$}
		\EndIf
		\EndFor
		\State{$\{\hat{\defVariable}_i:i\in\GroupTestItemSet\}=\GroupTest2(\GroupTestItemSet)$}
		\State{$\{\hat{\defVariable}_i:i\in\IndividualTestItemSet\}=\IndividualTest2(\IndividualTestItemSet)$}
		\State{\Return $\left[\hat{\defVariable}_1,\ldots,\hat{\defVariable}_\nItems\right]$}
	\end{algorithmic}
\end{algorithm}

==> algorithm-nonadaptive.tex <==
\begin{algorithm}
	\caption{Non-adaptive Community Testing ($\testmatrix_1,\testmatrix_2$)}
	\label{algorithm-nonadaptive} 
	$\testmatrix_1$ of size $\nTests_1\times \nItems$ is the upper part of the testing matrix that identifies the non-infected communities. \\
	$\testmatrix_2$ of size $\nTests_2\times \nItems$ is the lower part of the testing matrix that identifies the non-infected and infected members. \\
	$\testmatrixEntry_{l,i}$ is the element in the $l$-th row and $i$-th column of testing matrix $\testmatrix_2$ (0 or 1). \\
	$\Outcome()$ is the outcome of a group testing.\\
	$\GroupTest()$ gives the testing result of the group test. \\
	$\MemberInclusionSet(i)$ is the set of communities that include member $i$. \\
	$\hat{\FamilyTestResult}_i$ is the estimated infection status of community $i$ (1 for ``positive'' and 0 for ``negative'').\\
	$\hat{\defVariable}_\memberIndex$ is the estimated infection status of member $\memberIndex$ (1 for ``positive'' and 0 for ``negative'').
	\begin{algorithmic}[1]
		\State{$\left[\hat{\FamilyTestResult}_1,\cdots,\hat{\FamilyTestResult}_{\nTests_1}\right]=\GroupTest(\testmatrix_1)$}
		\State{$\left[\testOutcome_1,\cdots,\testOutcome_{\nTests_2}\right]=\Outcome(\testmatrix_2)$}
		\For {$i\in[1:\nItems]$}
		\If{$\sum(\hat{\FamilyTestResult}_j:~j\in\mathit{MemberInclusionSet}(i))==0$}
		\State{$\hat{\defVariable}_i=0$}
		\Else
		\For{$l\in[1:\nTests_2]$}
		\If{$(\testOutcome_l:~l\in[1:\nTests_2],\testmatrixEntry_{l,i}=1) == 0$}
		\State{$\hat{\defVariable}_i=0$}
		\Else
		\State{$\hat{\defVariable}_i=1$}
		\EndIf
		\EndFor
		\EndIf
		\EndFor
		
		\State{\Return $\left[\hat{\defVariable}_1,\ldots,\hat{\defVariable}_\nItems\right]$}
	\end{algorithmic}
\end{algorithm}


==> model-X.tex <==

\section{Notation}
\label{sec:model}
%==================================

\subsection{Community model}
\label{sec:notation:models}
\textcolor{blue}{Pavlo, the following definition for the hypergraph may be more natural, but not changing in the main file so that we dont lose consistency with other parts.}

In this paper, we assume that all \textit{members} of the entire population $\itemsSet = \{1,2,\cdots,\nItems\}$ are organized in a known \textit{community} structure, which can be conceived in the form of a hyper graph $\graph(\vertexSet,\edgeSet)$:  
each vertex $\vertexIndex \in \vertexSet$ corresponds to a member and an edge $\edgeIndex \in \edgeSet$ 
corresponds to a community (i.e. a group of members).

We use two functions to map sets of members to sets of communities and vice versa. 
For any subset of members $\setIdx$, 
$\memToFam (\setIdx)$ is the set of unique communities having at least one member in $\setIdx$. 
Additionally, for any subset of communities $\vertexSubset \subseteq \edgeSet$, 
$\famToMem (\vertexSubset)$ is the set of unique members that belong to all communities in $\vertexSubset$.
For example, 
$\famToMem(\edgeSet) = \itemsSet$,
$\memToFam(\itemsSet) = \edgeSet$, 
and when a set of communities $\vertexSubset$ overlap,
then this means: $\cap_{\vertexIndex \in \vertexSubset}\famToMem(\vertexIndex) \neq \emptyset$.

In our analysis, we need to decompose $\graph$ into a set of components, 
we denote this set with $\components_\graph$.
Since each component $\component \in \components_\graph$ is just a subset of vertices/communities, 
$\famToMem(\component)$ is the set of all members in that subset (the component). 
Also, $\disjointSets$ will denote the maximum-rank partition of $\famToMem(\component)$;
that is, the smallest family of subsets of members in $\famToMem(\component)$ that are pairwise disjoint.
Fig.~\ref{fig:structure} depicts an example structure having 2 disconnected components $\left\{\component_1, \component_2 \right\}$ and their maximum-rank partitions.\pavlos{add figure here...}

We also frequently need to reason about the number of communities in the structure and the community size (i.e. the number of members in a community).
Instead of the classic cardinality notation, we use the following for brevity:
$|\vertexSet| = \nFamilies$,
$|\famToMem(\vertexIndex)| = \nMembers$,
and $\nMembers = \nMembersSymmetric$ 
in the symmetric case where all communities have the same size.



\subsection{Infection models}
A community (resp.~component) that contains at least on infected member is called \textit{infected}. 
Let $\setDef(set)$ return the subset of infected elements of any \textit{set} of members, communities or components. 

We consider the following infection models, that parallel the ones in the traditional setup.\\
$\bullet$ {\bf Combinatorial Model (I).}  $\nDefFamilies$ of the communities have at least one infected member (we will call these {\em infected communities}). 
The rest of the communities have no infected members. 
Any combination of infected communities has the same chance of occurring. 
In each infected community, there are $\nDefMembers = |\setDef(\famToMem(\vertexIndex))|$ infected members, 
out of which $\nDefMembersOverlap = |\cap_{\vertexIndex \in \vertexSubset}\setDef\left(\famToMem\left(\vertexIndex\right)\right)|$ are shared with a subset of communities $\vertexSubset$ that it overlaps with
(i.e. $\vertexSubset$ is such that $\cap_{\vertexIndex \in \vertexSubset}\famToMem(\vertexIndex) \neq \emptyset$).\\ 
%In the symmetric case, $\nDefMembers = \nDefMembersSymmetric$ for all  $\familyIndex \in \vertexSet$. \\
$\bullet$ {\bf Probabilistic Model (II).} A community $\vertexIndex$ becomes infected with probability $\familyInfectRate$
i.i.d.~across the communities. 
If $\vertexIndex$ is infected, then its infection rate is $\memberInfectRate$;
that is, any member that belongs \textit{only} to community $\vertexIndex$ is infected with probability $\memberInfectRate$,
i.i.d.~across all members that belong only to $\vertexIndex$ and independently from other members, communities and components. 
A member of an infected community is infected, 
independently from the other members (and other communities), with probability $\memberInfectRateSymmetric_\memberIndex = \memberInfectRate$. The rest of the families have no infected members.
Additionally, a member that belongs to more than one communities is considered to be infected by either of the communities it belongs to;
that is, 
if member $\memberIndex$ participates in a subset of communities $\vertexSubset$ with $|\vertexSubset| > 1$ and infection rates $\left\{\memberInfectRate: \vertexIndex \in \vertexSubset\right\}$,
then $\memberIndex$ becomes infected independently from all other members with probability\footnote{The probability is the probability of the union of the infection events from either of the communities $\memberIndex$ participates in and follow the inclusion-exclusion principle.}:
\begin{equation}\label{eq:union-prob}
\memberInfectRateSymmetric_\memberIndex = \sum_{t = 1}^{|\vertexSubset|} \left(-1\right)^{t-1} \sum_{K \subseteq \vertexSubset, |K| = t} \memberInfectRateSymmetric_K,\; \text{ where }\; \memberInfectRateSymmetric_K = \prod_{\vertexIndex \in K} \memberInfectRate.
\end{equation}

\textcolor{blue}{Not sure we should keep either, removed for now.} 
%Our infection models capture situations where infection is determined by participation in the community rather than the status of the community members: the underlying assumption is that all community members start as healthy, but get exposed to infection through the community participation, for example because 
%there exist members that do not belong to $\itemsSet$, yet interact with them in ways that are unknown, 
%or there might be communities that are simply not captured by graph $\graph$ because of partial knowledge of member interactions.

%reflect well what will happen in practice. In the case of a pandemic, where a large number of people from different places and countries may be affected, 
%we cannot expect that the community structure of the entire population of a country of a continent is known to the group-test designer. 
%In fact, there might many members that do not belong to $\itemsSet$, yet interact with them in ways that are unknown, 
%or there might be communities that are simply not captured by graph $\graph$ because of partial knowledge of member interactions. 
%Hence, it is reasonable to assume that communities may become infected almost independently and model the infection of each community as a random event that happens with uniform probability. 
%However, once few communities become infected, 
%we expect that the probability of a member becoming infected should be a function of the communities it belongs to. 
%In this regard, eq.~\ref{eq:union-prob} shows the probability that an individual
%becomes infected by either of the infected communities it participates in. 


\subsection{Noisy testing and error probability} 

In this work we assume that there is no dilution noise. That is, the performance of a test does not depend on the number of samples pooled together. This is a reasonable assumption with genetic RT-PCR tests used in virus detection where the genetic material is ``amplified" and thus even small amounts of viral nucleotides can be amplified to be detectable \cite{Mullis85}.
%\footnote{In  such tests,  the genetic material is ``amplified" using the PCR techniques, whereby even small amounts of viral nucleotides can be amplified to be detectable \cite{Mullis85}. Therefore we can pool after sufficient amplification.}.

\pavlos{add more about the noisy testing model (e.g. define z-channel, false-negative, false-positive probabilities, etc.)}

==> noisy.tex <==
%============================================
\section{Testing with noise}\label{sec:Noisy-Testing}
%============================================
We have shown in \cite{GroupTesting-community} that leveraging community structure can improve the reliability when test outputs are noisy. 
Here we show similar results that taking overlap structure into account can further improve the reliability. 
Theoretical error analysis for a special community structure is given in this section, and numerical simulations are provided for more general cases in \Cref{section-experiments}. 

Assume that positive test outputs can flip with probability $\znoiseProb$, as illustrated by the Z-channel in Fig.~\ref{fig-Z}.
\begin{figure}[!h]
	\centering
	\begin{tikzpicture}
		\node at (-0.8,0.6) {$Y_\tau$}; \node at (2.8,0.6) {$\hat{Y}_\tau$}; 
		\draw[->,>=stealth] (0,0)--(2,0); \node[below] at (1,0) {$1-z$}; \node[left] at (0,0) {$1$}; \node[right] at (2,0) {$1$};
		\draw[-stealth,red] (0,0)--(2,1.2); \node[left] at (1.5,0.5) {$z$}; 
		\draw[-stealth] (0,1.2)--(2,1.2);   \node[left] at (0,1.2) {$0$}; \node[right] at (2,1.2) {$0$};
	\end{tikzpicture}
	\caption{Z-channel noise.}
	\label{fig-Z}
\end{figure}
To improve reliability, we consider the following: (1) group testing all members regardless of the community structure; (2) two stage algorithm leveraging the overlap structure. 
The comparison with a two-stage algorithm that takes community structure into account but do not take overlap into account is given in Appendix~\ref{app:sec:NoisyTesting}. 
\begin{enumerate}[(1)]
	\item {\bf Group testing.} We can view group testing as a form of coding, aiming to introduce redundancy to correct errors. 
	We consider constant weight designs of testing matrices $\testmatrix$, where each item is included in $L$ tests, chosen uniformly at random.
	For the threshold decision rule 
	\begin{equation}
		\hat{x}_i=
		\begin{cases}
			0,&\text{if }|\{t\in\mathcal{T}: \hat{y}_t=0,\testmatrixEntry_{t,i}=1\}|>\znoiseProb(1+\delta)L \\
			1,&\text{if }|\{t\in\mathcal{T}: \hat{y}_t=1,\testmatrixEntry_{t,i}=1\}|\geq (1-\znoiseProb(1+\delta))L, 
		\end{cases}  \label{Constant-threshold-decision-rule}
	\end{equation}
	we obtain from \cite{GroupTesting-community} that $\Pr(\text{FN}) \leq e^{-2L(\znoiseProb\delta)^2}$. 
	We simply choose $L=\frac{\nTests}{\nDef}$, then 
	\begin{equation}
		\Pr(\text{FN}) \leq e^{-\frac{2\nTests}{\nDef}(\znoiseProb\delta)^2}.   \label{FN-prob}
	\end{equation}
	
	
	\item {\bf Using overlap structure.} We adapt the two-stage algorithm Alg.~\ref{algorithm-2stage} and compare this against group testing. The algorithm is characterized as follows. 
	
	\textbf{Stage 1:} Group test pooled samples obtained from pooling all non-overlapped members in each community. 
	
%	\textbf{Classification of community members based on Stage 1:} 
	For any member $i$, if it is included in some infected community, then $i\in\IndividualTestItemSet$; otherwise, if all the communities that include $i$ are non-infected, then~$i\in\GroupTestItemSet$. 
	
	\textbf{Stage 2:} Perform group tests to $\GroupTestItemSet$ and individual tests to $\IndividualTestItemSet$. 
\end{enumerate}

\input{algorithm-2stage}

For performance analysis, we now consider a special community structure where each member is contained in at most two communities. 
The community structure can be represented by a graph where each vertex corresponds a community and two vertexes are connected if the corresponding communities have overlaps. 
An example of such community and its graph representation is illustrated in Fig.~\ref{fig-2overlap}. 
\begin{figure}[!h]
	\centering
	\begin{subfigure}{0.5\textwidth}
		\centering
		\begin{tikzpicture}[scale=0.6]
			\draw (-2.1,0) circle (1); \draw (-0.7,0) circle (1); \draw (0.7,0) circle (1); \draw (2.1,0) circle (1); 
			
			%			\def\testcircle{(0.3,1) .. controls (-2,1.5) and (-3,-5) .. (0,-5) .. controls (3,-5) and (0.5,-2.5) .. (0.3,-2).. controls (-0.5,-0.5) and (2.5,0.5) .. (0.3,1)}
			\def\5circle{(-1.0,-0.5) .. controls (-1.5,-3) and (1.5,-3) .. (1.0,-0.5) .. controls (0.8,0.5) and (0.5,-1.7) .. (0,-1.7).. controls (-0.5,-1.7) and (-0.8,0.5) .. (-1.0,-0.5) }
			
			\draw\5circle; 
		\end{tikzpicture}
		\vspace{-0.4cm}
		\caption{Community structure.}
		\label{fig-2overlap-structure}
	\end{subfigure}
	~
	\begin{subfigure}{0.45\textwidth}
		\centering
		\begin{tikzpicture}[scale=1.5]
			\filldraw (-0.5,0) circle (2pt); \filldraw (0,0) circle (2pt); \filldraw (0.5,0) circle (2pt); \filldraw (1.0,0) circle (2pt); \filldraw (0.25,-0.4) circle (2pt); 
			\draw (-0.5,0)--(0,0)--(0.5,0)--(1.0,0) (0,0)--(0.25,-0.4)--(0.5,0);
			
			\draw [white] (0,0.8) circle (2pt); 
		\end{tikzpicture}
		\caption{Graph representation.}
		\label{fig-2overlap-graph}
	\end{subfigure}
	\caption{Community structure example.}
	\label{fig-2overlap}
\end{figure}

Recall that $\nTests$ is the total number of tests. 
Let $\nTests_{1},\nTests_{2},\nTests_{3}$ be the number of tests in the two-stage algorithm for community testing, testing non-infected communities, and testing infected communities, respectively. 
Then the constant column weight used for stage 1 and group testing in stage 2 are $\frac{\nTests_1}{\nDefFamilies}$ and $\frac{\nTests_2}{\nDef_2}$, where $\nDef_2$ is the expected number of infected members in $\GroupTestItemSet$, and can be obtained as 
\begin{align}
	\nDef_2&=Q_{1}\nDefFamilies\nDefMembersSymmetric-N_{\text{infected in overlap}}\cdot\Pr(i\& j \text{ infected, } i \text{ or } j \text{ FN}|\text{communities } i, j\text{ overlap})  \\
	&=Q_{1}\nDefFamilies\nDefMembersSymmetric-N_{\text{infected in overlap}}\cdot\frac{\nDefFamilies(\nDefFamilies-1)}{F(F-1)}\cdot(2z(1-z))   \label{k-o2-prob}\\
	&\stackrel{sparse}{\approx}Q_{1}\nDefFamilies\nDefMembersSymmetric,   \label{k-o2}
\end{align}
where $N_{\text{infected in overlap}}$ is the average number of infected members in overlaps, 
and the first equality holds because almost all false negatives in stage 1 put $\nDefMembersSymmetric$ infected members into $\GroupTestItemSet$, except the false negatives that happens to only one of two infected overlapped communities, for which $\nDefMembersSymmetric-N_{\text{infected in overlap}}$ members are put into $\GroupTestItemSet$. 
For comparison, let $\nTests_1 + \nTests_2 + \nTests_{3} = T$. 
We use the following notations. 
\begin{align}
	Q &= \Pr(FN|\text{no community})   \\
	Q_{o} &= \Pr(FN|\text{overlap}) & Q_{1} &= \Pr(FN|\text{Stage 1, overlap})  \\
	Q_{2} &= \Pr(FN|\text{Test } \GroupTestItemSet, \text{ overlap}) & 
	Q_{3} &=\Pr(FN|\text{Test } \IndividualTestItemSet, \text{ overlap}). 
\end{align}
We want to compare $Q$ against $Q_o$, which can be obtained as $Q_o=Q_{1}Q_{2}+(1-Q_{1})Q_{3}$. 
We consider the case where $\nDefMembersSymmetric \approx \nMembersSymmetric$, i.e., almost all members of an infected community are infected; we can then choose to label all members in $\IndividualTestItemSet$ as infected. 
In such a case $Q_{3}=0$, at the cost of a slight increase in false positive probability. 
From the FN probability for group testing in \eqref{FN-prob}, we have 
\begin{align}
	&Q\leq \exp\left[-\frac{2\nTests}{\nDefFamilies \nDefMembersSymmetric}(\znoiseProb\delta)^2\right],\quad Q_{1}\leq \exp\left[-\frac{2\nTests_1}{\nDefFamilies}(\znoiseProb\delta)^2\right], Q_{2}\leq \exp\left[-\frac{2\nTests_2}{Q_{1}\nDefFamilies \nDefMembersSymmetric}(\znoiseProb\delta)^2\right].  \label{Q-bound-overlap}
\end{align}
Now we obtain 
\begin{align}
	Q_o&\approx Q_{1}Q_{2}\leq Q_{1}\leq e^{-\frac{2\nTests_1}{\nDefFamilies}(\znoiseProb\delta)^2}= \left(e^{-\frac{2\nTests}{\nDefFamilies\nDefMembersSymmetric}(\znoiseProb\delta)^2}\right) ^{\frac{\nTests_1\nDefMembersSymmetric}{T}}, \label{compare-overlap-GT}
\end{align}
which suggests that for $\nTests_1=c\nTests$ with $c$ a constant, the upper bound for $Q_{o}= \Pr(FN|\text{overlap})$ can be exponentially smaller than the upper bound for $Q= \Pr(FN|\text{no community})$. 


